Recognition of Unseen Bird Species by Learning from Field Guides

We exploit field guides to learn bird species recognition, in particular zero-shot recognition of unseen species. Illustrations contained in field guides deliberately focus on discriminative properties of each species, and can serve as side information to transfer knowledge from seen to unseen bird species. We study two approaches: (1) a contrastive encoding of illustrations, which can be fed into standard zero-shot learning schemes; and (2) a novel method that leverages the fact that illustrations are also images and as such structurally more similar to photographs than other kinds of side information. Our results show that illustrations from field guides, which are readily available for a wide range of species, are indeed a competitive source of side information for zero-shot learning. On a subset of the iNaturalist2021 dataset with 749 seen and 739 unseen species, we obtain a classification accuracy of unseen bird species of $12\%$ @top-1 and $38\%$ @top-10, which shows the potential of field guides for challenging real-world scenarios with many species. Our code is available at https://github.com/ac-rodriguez/zsl_billow

==> tables/mbank_cub_backbones_results-may.tex <==
\begin{tabular}{lrrr}
\hline
% Backbone &    H &    S &    U \\
% \hline
% Resnet-18  & 42.0 & 48.2 & 37.2 \\
% Resnet-50  & 47.8 & 64.8 & 37.8 \\
% Resnet-101 & 47.5 & 69.7 & 36.1 \\

Backbone &   S &    U & H  \\
\hline
Resnet-18   & 48.2 & 37.2  & 42.0\\
Resnet-50   & 64.8 & 37.8& 47.8 \\
Resnet-101  & 69.7 & 36.1 & 47.5\\

\hline
\end{tabular}

